Think Deep, Not Just Long: Measuring LLM Reasoning Effort via Deep-Thinking Tokens

Large language models (LLMs) have demonstrated impressive reasoning capabilities by scaling test-time compute via long Chain-of-Thought (CoT). However, recent findings suggest that raw token counts are unreliable proxies for reasoning quality: increased generation length does not consistently correlate with accuracy and may instead signal "overthinking," leading to performance degradation. In this work, we quantify inference-time effort by identifying deep-thinking tokens -- tokens where internal predictions undergo significant revisions in deeper model layers prior to convergence. Across four challenging mathematical and scientific benchmarks (AIME 24/25, HMMT 25, and GPQA-diamond) and a diverse set of reasoning-focused models (GPT-OSS, DeepSeek-R1, and Qwen3), we show that deep-thinking ratio (the proportion of deep-thinking tokens in a generated sequence) exhibits a robust and consistently positive correlation with accuracy, substantially outperforming both length-based and confidence-based baselines. Leveraging this insight, we introduce Think@n, a test-time scaling strategy that prioritizes samples with high deep-thinking ratios. We demonstrate that Think@n matches or exceeds standard self-consistency performance while significantly reducing inference costs by enabling the early rejection of unpromising generations based on short prefixes.

==> algos/algo.tex <==
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \begin{algorithm}[t]
% \small
% \caption{Computing Deep-Thinking Ratio (DTR)}
% \label{alg:dtr}
% \begin{algorithmic}[1]
% \REQUIRE Autoregressive LM $f_\theta$ with $L$ layers and unembedding matrix $W_U$; Input prompt $x$; Threshold $g$; Depth fraction $\rho$
% \ENSURE $\mathrm{DTR}(S)$ of the generated sequence $S$

% \STATE $C \leftarrow 0,\; S \leftarrow \emptyset$
% \WHILE{not stop}
%   \STATE Sample $y_t \sim p_{t,L}\!\left(f_\theta(\cdot \mid x,S)\right)$
%   \STATE $S \leftarrow (S,y_t)$
%   \FOR{$l=1$ {\bf to} $L$}
%     \STATE $p_{t,l} \leftarrow \mathrm{softmax}(W_U h_{t,l})$
%   \ENDFOR
%   \STATE $D_{t,l} \leftarrow \mathrm{JSD}(p_{t,l},p_{t,L})\;\forall l$
%   \STATE $c_t \leftarrow \min\{l:\min_{j\le l} D_{t,j} \le g\}$
%   \IF{$c_t \ge \lceil(1-\rho)L\rceil$}
%     \STATE $C \leftarrow C+1$
%   \ENDIF
% \ENDWHILE

% \STATE \textbf{return} $C/|S|$
% \end{algorithmic}
% \end{algorithm}

% In preamble:
% \usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\begin{algorithm}[t]
\small
\caption{Computing Deep-Thinking Ratio (DTR)}
\label{alg:dtr}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Autoregressive LM $f_\theta$ with $L$ layers and unembedding matrix $W_U$; Input prompt $x$; Threshold $g$; Depth fraction $\rho$}
\Output{$\mathrm{DTR}(S)$ of the generated sequence $S$}

$C \leftarrow 0,\; S \leftarrow \emptyset$\;
\While{not stop}{
  Sample $y_t \sim p_{t,L}\!\left(f_\theta(\cdot \mid x,S)\right)$\;
  $S \leftarrow (S,y_t)$\;
  \For{$l \leftarrow 1$ \KwTo $L$}{
    $p_{t,l} \leftarrow \mathrm{softmax}(W_U h_{t,l})$\;
  }
  $D_{t,l} \leftarrow \mathrm{JSD}(p_{t,l},p_{t,L})\;\forall l$\;
  $c_t \leftarrow \min\{l:\min_{j\le l} D_{t,j} \le g\}$\;
  \If{$c_t \ge \lceil(1-\rho)L\rceil$}{
    $C \leftarrow C+1$\;
  }
}
\Return $C/|S|$\;

\end{algorithm}
